A Step Towards Worldwide Biodiversity Assessment: The BIOSCAN-1M Insect Dataset

In an effort to catalog insect biodiversity, we propose a new large dataset of hand-labelled insect images, the BIOSCAN-Insect Dataset. Each record is taxonomically classified by an expert, and also has associated genetic information including raw nucleotide barcode sequences and assigned barcode index numbers, which are genetically-based proxies for species classification. This paper presents a curated million-image dataset, primarily to train computer-vision models capable of providing image-based taxonomic assessment, however, the dataset also presents compelling characteristics, the study of which would be of interest to the broader machine learning community. Driven by the biological nature inherent to the dataset, a characteristic long-tailed class-imbalance distribution is exhibited. Furthermore, taxonomic labelling is a hierarchical classification scheme, presenting a highly fine-grained classification problem at lower levels. Beyond spurring interest in biodiversity research within the machine learning community, progress on creating an image-based taxonomic classifier will also further the ultimate goal of all BIOSCAN research: to lay the foundation for a comprehensive survey of global biodiversity. This paper introduces the dataset and explores the classification task through the implementation and analysis of a baseline classifier.

==> macros.tex <==
% if you need to pass options to natbib, use, e.g.:
\PassOptionsToPackage{numbers, compress}{natbib}
% before loading neurips_data_2022

% ready for submission
% if you need to pass options to natbib, use, e.g.:
%     \PassOptionsToPackage{numbers, compress}{natbib}
% before loading neurips_data_2023

% camera-ready
\usepackage[final]{neurips_data_2023}

% to compile a preprint version, add the [preprint] option, e.g.:
%     \usepackage[preprint]{neurips_data_2023}
% This will indicate that the work is currently under review.

% to compile a camera-ready version, add the [final] option, e.g.:
%     \usepackage[final]{neurips_data_2023}

% to avoid loading the natbib package, add option nonatbib:
%    \usepackage[nonatbib]{neurips_data_2023}

% Submissions to the datasets and benchmarks are typically non anonymous,
% but anonymous submissions are allowed. If you feel that you must submit 
% anonymously, you can compile an anonymous version by adding the [anonymous] 
% option, e.g.:
%     \usepackage[anonymous]{neurips_data_2023}
% This will hide all author names.

\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{xcolor}         % colors

%%%% INCLUDE PACKAGES
\usepackage{array}
\usepackage{amsmath}
\usepackage{makecell}
\usepackage{multirow}
\usepackage{graphicx}
\usepackage{subcaption}
\captionsetup{compatibility=false}
\usepackage{geometry}
\usepackage{comment}
\usepackage{floatrow}
\usepackage{wrapfig}	
\usepackage{tabularx}
\renewcommand\tabularxcolumn[1]{m{#1}}% for vertical centering text in X column
\newcolumntype{Y}{>{\centering\arraybackslash}X}

\usepackage{booktabs}
\usepackage{floatrow}
\floatsetup[table]{capposition=top}
\setlength{\belowcaptionskip}{-10pt}
%\usepackage[tableposition=top]{caption}
%\usepackage{float}
%\floatstyle{plaintop}
%\restylefloat{table}
\usepackage{makecell}
\setlength{\textfloatsep}{5.0pt plus 5.0pt minus 2.0pt}
\usepackage{titlesec}
\titlespacing\section{1pt}{1pt}{1pt}
\titlespacing\subsection{1pt}{1pt}{1pt}
\titlespacing\subsubsection{1pt}{1pt}{1pt}
\titlespacing\paragraph{1pt}{1pt}{1pt}
\usepackage[capitalize,noabbrev]
{cleveref}

% \usepackage{siunitx}     % typeset units (temporarily disabled)
% \sisetup{detect-all}     % don't switch fonts when typesetting numbers

%%%% OUR MACROS

\newcommand{\graham}[1]{\textcolor{blue}{[Graham: #1]}}
\newcommand{\paul}[1]{\textcolor{ForestGreen}{[Paul: #1]}}
\newcommand{\angel}[1]{\textcolor{orange}{[Angel: #1]}}
\newcommand{\iuliia}[1]{\textcolor{Plum}{[Iuliia: #1]}}
\newcommand{\zahra}[1]{\textcolor{magenta}{[Zahra: #1]}}
\newcommand{\nick}[1]{\textcolor{cyan}{[Nick: #1]}}
\newcommand{\ming}[1]{\textcolor{brown}{[Ming: #1]}}

\newcommand{\todo}[1]{\textcolor{red}{[Todo: #1]}}
% Highlighting stuff that's changed in the revision
\newcommand{\revised}[1]{{\leavevmode\color{teal}#1}}
% \newcommand{\revised}[1]{#1}
\newcommand{\added}[1]{{\leavevmode\color{blue}#1}}


\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\orange}[1]{\textcolor{orange}{#1}}

\usepackage{xspace}
\newcommand{\eg}{e.g.,\xspace}
\newcommand{\ie}{i.e.,\xspace}


\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}
\def\etal{\emph{et al}\onedot}
\def\aka{\emph{aka}\ }
\def\etc{\emph{etc}\onedot} 
\def\vs{\emph{vs}\onedot}
\makeatother

\usepackage{enumitem}

\newcommand{\ctab}[1]{\begin{tabular}{c}#1\end{tabular}}
\newcommand{\ltab}[1]{\begin{tabular}{l}#1\end{tabular}}
